Lexicosyntactic Inference in Neural Models

We investigate neural models' ability to capture lexicosyntactic inferences: inferences triggered by the interaction of lexical and syntactic information. We take the task of event factuality prediction as a case study and build a factuality judgment dataset for all English clause-embedding verbs in various syntactic contexts. We use this dataset, which we make publicly available, to probe the behavior of current state-of-the-art neural systems, showing that these systems make certain systematic errors that are clearly visible through the lens of factuality prediction.

==> tables/badpredictions.tex <==
\begin{tabular}{lrr}
\toprule
                        Sentence &  True &  Predicted \\
\midrule
           someone faked that something happened . &       -3.15 &       0.86 \\
 someone was misinformed that something happened . &       -2.62 &       1.37 \\
               someone neglected to do something . &       -3.07 &      -0.02 \\
             someone pretended to have something . &       -2.96 &       0.05 \\
         someone was misjudged to have something . &       -2.46 &       0.55 \\
                someone forgot to have something . &       -3.18 &      -0.17 \\
             someone neglected to have something . &       -2.93 &       0.07 \\
       someone pretended that something happened . &       -2.11 &       0.86 \\
                someone declined to do something . &       -3.18 &      -0.22 \\
             someone was refused to do something . &       -3.16 &      -0.22 \\
                 someone refused to do something . &       -3.12 &      -0.20 \\
               someone pretended to do something . &       -3.02 &      -0.11 \\
      someone disallowed someone to do something . &       -2.56 &       0.34 \\
          someone was declined to have something . &       -2.36 &       0.55 \\
              someone declined to have something . &       -3.12 &      -0.23 \\
      someone did n't hesitate to have something . &        1.84 &      -0.96 \\
                someone ceased to have something . &       -2.22 &       0.57 \\
        someone did n't hesitate to do something . &        1.86 &      -0.92 \\
            someone lied that something happened . &       -1.99 &       0.78 \\
               someone feigned to have something . &       -3.07 &      -0.31 \\
%           someone did n't forget to do something . &        1.84 &      -0.92 \\
%          someone refused someone to do something . &       -2.65 &       0.09 \\
%          someone did n't neglect to do something . &        1.86 &      -0.86 \\
%                   someone forgot to do something . &       -2.81 &      -0.13 \\
%             someone did n't mean to do something . &        1.87 &      -0.81 \\
\bottomrule
\end{tabular}

==> tables/corr_by_frame.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{c}{Linear} & \multicolumn{2}{c}{Tree} & \multicolumn{2}{c}{Hybrid} \\
 & pos & neg & pos & neg & pos & neg \\
\midrule
NP \_ed that S         &     \textbf{0.25} &    -0.02 &     0.19 &     \textbf{0.12} &     0.19 &     0.10 \\
NP was \_ed that S     &     0.11 &     0.20 &     0.08 &     0.17 &     \textbf{0.23} &     \textbf{0.24} \\
NP \_ed for NP to VP   &     \textbf{0.26} &    \textbf{-0.02} &    -0.00 &    -0.06 &    -0.00 &    -0.04 \\
NP \_ed NP to VP[+ev]  &    -0.04 &    -0.20 &     \textbf{0.04} &     0.20 &    -0.08 &     \textbf{0.22} \\
NP \_ed NP to VP[-ev]  &    -0.09 &    -0.01 &     \textbf{0.00} &     \textbf{0.24} &    -0.08 &     0.16 \\
NP was \_ed to VP[+ev] &     0.21 &     0.24 &     \textbf{0.29} &     0.38 &     0.26 &     \textbf{0.41} \\
NP was \_ed to VP[-ev] &     0.36 &     0.13 &     \textbf{0.44} &     0.43 &     0.40 &     \textbf{0.55} \\
NP \_ed to VP[+ev]     &     0.09 &     0.14 &     \textbf{0.20} &     \textbf{0.23} &    -0.06 &     0.02 \\
NP \_ed to VP[-ev]     &     0.24 &     0.13 &     \textbf{0.25} &     \textbf{0.22} &     0.12 &     0.06 \\
\bottomrule
\end{tabular}

==> tables/correlations.tex <==
\begin{tabular}{lllrrr}
\toprule
 biLSTM &   Dataset &  UNK &  Raw &  Freq. weight &  Acc. weight\\
\midrule
 Linear &       UDS &  False &        0.48 &            0.41 &           0.48 \\
 Linear &        UW &  False &        0.55 &            0.51 &           0.55 \\
 Linear &  MEANTIME &  False &        0.47 &            0.44 &           0.49 \\
 Linear &  FactBank &  False &        0.44 &            0.40 &           0.45 \\
   Tree &       UDS &  False &        0.56 &            0.53 &           0.56 \\
   Tree &        UW &  False &        0.53 &            0.53 &           0.54 \\
   Tree &  MEANTIME &  False &        0.44 &            0.48 &           0.47 \\
   Tree &  FactBank &  False &        0.52 &            0.52 &           0.53 \\
 Hybrid &       UDS &  False &        0.53 &            0.47 &           0.53 \\
 Hybrid &        UW &  False &        0.32 &            0.33 &           0.34 \\
 Hybrid &  MEANTIME &  False &        0.03 &            0.05 &           0.06 \\
 Hybrid &  FactBank &  False &        0.24 &            0.25 &           0.27 \\
 \midrule
 Linear &       UDS &   True &        0.40 &            0.32 &           0.42 \\
 Linear &        UW &   True &        0.51 &            0.50 &           0.51 \\
 Linear &  MEANTIME &   True &        0.44 &            0.44 &           0.45 \\
 Linear &  FactBank &   True &        0.43 &            0.43 &           0.42 \\
   Tree &       UDS &   True &        0.22 &            0.11 &           0.26 \\
   Tree &        UW &   True &        0.53 &            0.53 &           0.51 \\
   Tree &  MEANTIME &   True &        0.36 &            0.40 &           0.31 \\
   Tree &  FactBank &   True &        0.50 &            0.51 &           0.48 \\
 Hybrid &       UDS &   True &        0.48 &            0.43 &           0.47 \\
 Hybrid &        UW &   True &        0.23 &            0.22 &           0.26 \\
 Hybrid &  MEANTIME &   True &       -0.09 &           -0.07 &          -0.08 \\
 Hybrid &  FactBank &   True &        0.03 &           -0.00 &           0.09 \\
 \midrule
 \multicolumn{3}{c}{Ensembled (CVed ridge regression)} & 0.59 & 0.56 & 0.57 \\
\bottomrule
\end{tabular}

==> tables/framecounts.tex <==
\begin{tabular}{lrll}
\toprule
Frame &  \# verbs & Ex. & Source \\
\midrule
NP \_ed that S         &       375 & \ref{ex:finiteintrans} & \citep{white_role_2018} \\
NP was \_ed that S     &       169 & \ref{ex:finitetrans} & \citep{white_role_2018} \\
NP \_ed for NP to VP   &       184 & \ref{ex:forto} & this paper \\
NP \_ed NP to VP[+ev]  &       197 & \ref{ex:aci_eventive} & this paper \\
NP \_ed NP to VP[-ev]  &       128 & \ref{ex:aci_stative} & this paper \\
NP was \_ed to VP[+ev] &       278 & \ref{ex:infinitivalpassive_eventive} & this paper \\
NP was \_ed to VP[-ev] &       256 & \ref{ex:infinitivalpassive_stative} & this paper \\
NP \_ed to VP[+ev]     &       217 & \ref{ex:control_eventive} & this paper \\
NP \_ed to VP[-ev]     &       165 & \ref{ex:control_stative} & this paper \\
\midrule
Total                  &       1,969 & \\
\bottomrule
\end{tabular}
